On-Manifold Preintegration for Real-Time Visual-Inertial Odometry

Current approaches for visual-inertial odometry (VIO) are able to attain highly accurate state estimation via nonlinear optimization. However, real-time optimization quickly becomes infeasible as the trajectory grows over time, this problem is further emphasized by the fact that inertial measurements come at high rate, hence leading to fast growth of the number of variables in the optimization. In this paper, we address this issue by preintegrating inertial measurements between selected keyframes into single relative motion constraints. Our first contribution is a \emph{preintegration theory} that properly addresses the manifold structure of the rotation group. We formally discuss the generative measurement model as well as the nature of the rotation noise and derive the expression for the \emph{maximum a posteriori} state estimator. Our theoretical development enables the computation of all necessary Jacobians for the optimization and a-posteriori bias correction in analytic form. The second contribution is to show that the preintegrated IMU model can be seamlessly integrated into a visual-inertial pipeline under the unifying framework of factor graphs. This enables the application of incremental-smoothing algorithms and the use of a \emph{structureless} model for visual measurements, which avoids optimizing over the 3D points, further accelerating the computation. We perform an extensive evaluation of our monocular \VIO pipeline on real and simulated datasets. The results confirm that our modelling effort leads to accurate state estimation in real-time, outperforming state-of-the-art approaches.

==> figureBiasConvergence.tex <==
\begin{figure}[t!]
  \centering
  \hspace{-5mm}
  \includegraphics[width=1.4\linewidth,trim = 0mm 50mm 0mm 0mm, clip]{\figdirvin/gray}
  \caption{Bias convergence.
  }
  \label{fig:bias_convergence}
  \vspace{-10px}
\end{figure}

==> figureBiasUpdate.tex <==
%!TEX root = main.tex

\begin{figure}[t!]
  \centering
  \includegraphics[width=1\linewidth]{\figdirvin/synthetic/vin_bias_acc.png}
  \vspace{-10px}
  \includegraphics[width=1\linewidth]{\figdirvin/synthetic/vin_bias_gyro.png}
  \caption{The simulated acceleration and gyroscope measurements are corrupted by a time varying bias modelled according to \Equation~\eqref{eq:discreteBias}. The blue lines show the bias estimated by the estimator at every time instant.}
  \label{fig:synthetic_bias}
  \vspace{-15pt}
\end{figure}
